SELECT: A Large-Scale Benchmark of Data Curation Strategies for Image Classification

Data curation is the problem of how to collect and organize samples into a dataset that supports efficient learning. Despite the centrality of the task, little work has been devoted towards a large-scale, systematic comparison of various curation methods. In this work, we take steps towards a formal evaluation of data curation strategies and introduce SELECT, the first large-scale benchmark of curation strategies for image classification. In order to generate baseline methods for the SELECT benchmark, we create a new dataset, ImageNet++, which constitutes the largest superset of ImageNet-1K to date. Our dataset extends ImageNet with 5 new training-data shifts, each approximately the size of ImageNet-1K itself, and each assembled using a distinct curation strategy. We evaluate our data curation baselines in two ways: (i) using each training-data shift to train identical image classification models from scratch (ii) using the data itself to fit a pretrained self-supervised representation. Our findings show interesting trends, particularly pertaining to recent methods for data curation such as synthetic data generation and lookup based on CLIP embeddings. We show that although these strategies are highly competitive for certain tasks, the curation strategy used to assemble the original ImageNet-1K dataset remains the gold standard. We anticipate that our benchmark can illuminate the path for new methods to further reduce the gap. We release our checkpoints, code, documentation, and a link to our dataset at https://github.com/jimmyxu123/SELECT.

==> algorithms/sgd-algo.tex <==
\begin{algorithmic}
\REQUIRE $\theta_{\text{init}}, \theta_{0\text{init}}, \eta, \epsilon$
\STATE $\theta^{(0)} \gets \theta_{\text{init}}$
\STATE $\theta_0^{(0)} \gets \theta_{0\text{init}}$
\STATE $t \gets 0$
\REPEAT
\STATE $t \gets t + 1$
\STATE $\theta^{(t)} \gets \theta^{(t-1)} - \eta \left( \frac{1}{n} \sum_{i=1}^n \left( \texttt{SOFTMAX} \left( \theta^{(t-1)T} x^{(i)} + \theta_0^{(t-1)} \right) - y^{(i)} \right) x^{(i)} + 2\lambda \theta^{(t-1)} \right)$
\STATE $\theta_0^{(t)} \gets \theta_0^{(t-1)} - \eta \left( \frac{1}{n} \sum_{i=1}^n \left( \texttt{SOFTMAX} \left( \theta^{(t-1)T} x^{(i)} + \theta_0^{(t-1)} \right) - y^{(i)} \right) \right)$
\UNTIL{$| L(\theta^{(t)}, \theta_0^{(t)}) - L(\theta^{(t-1)}, \theta_0^{(t-1)}) | < \epsilon$}
\RETURN $\theta^{(t)}, \theta_0^{(t)}$
\end{algorithmic}

==> plots/H-scaling100.tex <==
% This file was created with tikzplotlib v0.10.1.

\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkred}{RGB}{139,0,0}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}
%\definecolor{blue}{RGB}{0,0,128}

\def\discon{$\wr\!\!\!\wr$}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1.0,0.35)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Data Budget (1x = 120,000 samples)},
xmajorgrids,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Accuracy/Average Robustness},
ymajorgrids,
ytick style={color=black},
xlabel style={font=\normalsize},
ylabel style={font=\normalsize},
width=16cm,
height=9cm,
xtick={0, 1, 2, 3, 4, 5, 6}, %edit for number for x-labels
ytick={0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0},
xticklabels={$1\times$, $2\times$, $4\times$, $5\times$, $10\times$, $20\times$, $1000\times$},
extra x ticks = {7.5},
extra x tick style  = {grid=none, xticklabel style={yshift=3.5mm, inner sep=.5pt}},
extra x tick labels = {\discon},
]
\addlegendentry{Baseline Val. Acc.}
\addplot [only marks, mark=*, mark size=3.0, draw=black, mark options={fill=black}]
table{
    x y
    0.0 0.853
};
\addlegendentry{Baseline Avg. Rob.}
\addplot [only marks, mark=triangle*, mark size=4.0, draw=black, mark options={fill=black}]
table{
    x y
    0.0 0.406
};
\addlegendentry{H-Scaling  Val. Acc.}
\addplot [only marks, mark=*, mark size=3.0, draw=blue, mark options={fill=blue}]
table{
    x y
    1.0 0.879
    1.0 0.882
    1.0 0.884
    1.0 0.883
    4.0 0.904
    4.0 0.907

};
\addlegendentry{H-Scaling  Val. Acc. (pretrained)}
\addplot [only marks, mark=o, mark size=3.0, draw=blue, mark options={fill=blue}]
table{
    x y
    4.0 0.952
    4.0 0.950
    5.1 0.958
};
\addlegendentry{H-Scaling Avg. Rob.}
\addplot [only marks, mark=triangle*, mark size=4.0, draw=blue, mark options={fill=blue}]
table{
    x y
    1.0 0.448
    1.0 0.455
    1.0 0.454
    1.0 0.457
    4.0 0.462
    4.0 0.468
};
\addlegendentry{H-Scaling Avg. Rob. (pretrained)}
\addplot [only marks, mark=triangle, mark size=4.0, draw=blue, mark options={fill=blue}]
table{
    x y
    4.0 0.522
    4.0 0.537
    5.1 0.59
};
\addlegendentry{V-Scaling  Val. Acc.}
\addplot [only marks, mark=*, mark size=3.0, draw=red, mark options={fill=red}]
table{
    x y
    1.0 0.897
    1.0 0.901
    1.0 0.904
    1.0 0.904
    1.0 0.904
    1.0 0.904
    2.0 0.908
    2.0 0.908
    2.0 0.917
    2.0 0.916
    2.0 0.917
    2.7 0.925
    2.7 0.927
    2.7 0.927
    %8.8 0.92
};
\addlegendentry{V-Scaling Avg. Rob.}
\addplot [only marks, mark=triangle*, mark size=4.0, draw=red, mark options={fill=red}]
table{
    x y
    1.0 0.508
    1.0 0.511
    1.0 0.512
    1.0 0.514
    1.0 0.517
    2.0 0.656
    2.0 0.664
    2.0 0.666
    2.0 0.672
    2.0 0.674
    2.7 0.689
    2.7 0.701
    2.7 0.702
    %8.8 0.76
};
\end{axis}


\end{tikzpicture}


==> plots/IN++Hscaling.tex <==
% This file was created with tikzplotlib v11.

\begin{tikzpicture}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkred}{RGB}{139,0,0}
\definecolor{green}{RGB}{0,128,0}
\definecolor{blue204}{RGB}{200,200,250}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{blue128}{RGB}{100,100,190}
\definecolor{lightgray128}{RGB}{128,128,128}
\definecolor{blue90}{RGB}{60,60,160}
\definecolor{green204}{RGB}{200,250,200}
\definecolor{green170}{RGB}{160,220,160}
\definecolor{green128}{RGB}{100,190,100}
\definecolor{green90}{RGB}{60,160,60}
\definecolor{green60}{RGB}{45,120,45}
\definecolor{green40}{RGB}{30,90,30}
%\definecolor{blue}{RGB}{0,0,128}

\def\discon{$\wr\!\!\!\wr$}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1.0,0.45)},
  anchor=north west,
  draw=lightgray204,
  font=\tiny,
  %text width=300pt,
},
xmin=60, xmax=85,
ymin=25, ymax=50,
tick align=outside,
tick pos=left,
tick label style={font=\tiny},
x grid style={lightgray204},
ylabel={IN1000 Avg. Rob.},
ylabel style={font=\tiny},
xmajorgrids,
y grid style={lightgray204},
xlabel={IN1000 Val. Acc.},
xlabel style={font=\tiny},
ymajorgrids,
]

% %upper CI
% \addplot [name path=upper, domain=60:85, samples=2, blue128, forget plot, draw=none] {1.16*x - 54.67};

% %best-fit line for V-scaling
% \addplot [domain=60:85, samples=2, blue128, line width=2, forget plot] {1.16*x - 54.67}; % y = 2x + 1

% %lower CI
% \addplot [name path=lower, domain=60:85, samples=2, blue128, forget plot, draw=none] {1.16*x - 54.67};


% %best-fit line for H-scaling
% \addplot [domain=60:85, samples=2, green128, line width=2, forget plot] {1.01*x - 38.32 }; % y = 2x + 1

%BASELINE
\addplot [only marks, mark=square*, mark size=2.0, draw=black, mark options={fill=lightgray128}]
table{
    x y
    77.9 33.4
};
\addlegendentry{Baseline}


%HSCALING
\addplot [only marks, mark=*, mark size=3.0, draw=black, mark options={fill=green128}]
table{
    x y
    69.2 31.0
};
\addplot [only marks, mark=*, mark size=3.5, draw=black, mark options={fill=green128},forget plot]
table{
    x y
    72.7 35.6
};
\addlegendentry{H-Scaling}

\addplot [only marks, mark=otimes*, mark size=3.0, draw=black, mark options={fill=green128},forget plot]
table{
    x y
    73.0 33.3
};

\addplot [only marks, mark=otimes*, mark size=3.5, draw=black, mark options={fill=green128}]
table{
    x y
    76.5 37.1
};
\addlegendentry{H-Scaling (fine-tuned)}

%VSCALING
\addplot [only marks, mark=triangle*, mark size=3.0, draw=black, mark options={fill=blue128}]
table{
    x y
    74.7 31.0
    77.1 35.7
    69.7 26.7
};
\addlegendentry{V-Scaling}

% \addlegendimage{empty legend}
% \addlegendentry{(Larger markers $->$ more data)}

\end{axis}


\end{tikzpicture}

==> plots/VandHscaling.tex <==

\begin{tikzpicture}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkred}{RGB}{139,0,0}
\definecolor{green}{RGB}{0,128,0}
\definecolor{blue204}{RGB}{200,200,250}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{blue128}{RGB}{100,100,190}
\definecolor{lightgray128}{RGB}{128,128,128}
\definecolor{blue90}{RGB}{60,60,160}
\definecolor{green204}{RGB}{200,250,200}
\definecolor{green170}{RGB}{160,220,160}
\definecolor{green128}{RGB}{100,190,100}
\definecolor{green90}{RGB}{60,160,60}
\definecolor{green60}{RGB}{45,120,45}
\definecolor{green40}{RGB}{30,90,30}
%\definecolor{blue}{RGB}{0,0,128}

\def\discon{$\wr\!\!\!\wr$}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1.0,0.45)},
  anchor=north west,
  draw=lightgray204,
  font=\tiny,
  %text width=300pt,
},
xmin=84, xmax=97,
ymin=37, ymax=73,
tick align=outside,
tick pos=left,
tick label style={font=\tiny},
x grid style={lightgray204},
ylabel={IN100 Avg. Rob.},
ylabel style={font=\tiny},
xmajorgrids,
y grid style={lightgray204},
xlabel={IN100 Val. Acc.},
xlabel style={font=\tiny},
ymajorgrids,
]

%upper CI
\addplot [name path=upper, domain=84:97, samples=2, blue128, forget plot, draw=none] {3.904*x + -295.7};

%best-fit line for V-scaling
\addplot [domain=84:97, samples=2, blue128, line width=2, forget plot] {3.904*x + -293.7}; % y = 2x + 1

%lower CI
\addplot [name path=lower, domain=84:97, samples=2, blue128, forget plot, draw=none] {3.904*x + -291.7};


%best-fit line for H-scaling
\addplot [domain=84:97, samples=2, green128, line width=2, forget plot] {1.442*x + -82.63}; % y = 2x + 1

% \addplot [blue!30] fill between[of=upper and lower];

% %RN26
% \addplot [only marks, mark=square*, mark size=3.0, draw=black, mark options={fill=lightgray204}, forget plot]
% table{
%     x y
%     81 40.3
% };
%RN50
\addplot [only marks, mark=square*, mark size=3.0, draw=black, mark options={fill=lightgray128}]
table{
    x y
    85.3 40.6
};
\addlegendentry{Baseline}

% %RN50x4
% \addplot [only marks, mark=square*, mark size=3.0, draw=black, mark options={fill=black}, forget plot]
% table{
%     x y
%     87.4 42.5
% };

%TODO: RN26 @ IN200, RN26 @ IN1000, RN50x4 @ IN200, RN50x4 @ IN1000

%RN50 IN200 H-sc
\addplot [only marks, mark=*, mark size=2.5, draw=black, mark options={fill=green128}]
table{
    x y
    87.9 44.8
    88.2 45.5
    88.4 45.4
    88.3 45.7
};
\addlegendentry{H-Scaling}

%RN50 IN1000 H-Sc (ours)
\addplot [only marks, mark=*, mark size=3.0, draw=black, mark options={fill=green128}, forget plot]
table{
    x y
    90.4 46.2
    
    90.7 46.8 
};

%RN50 IN1000 H-Sc (resnetv2_50.a1h_in1k)
% \addplot [only marks, mark=otimes*, mark size=3.0, draw=black, mark options={fill=green128}]
% table{
%     x y
%     95.2 52.2 
% };
% \addlegendentry{H-Scaling (from pretrained)}

%RN50 IN1000 ft 12000 32ep H-Sc (resnetv2_50.a1h_in1k)
% \addplot [only marks, mark=otimes*, mark size=3.5, draw=black, mark options={fill=green128}, forget plot]
% table{
%     x y
%     95.0 53.7
% };

%RN50 IN21000 ft 1000 zs 100 H-Sc (resnetv2_50.a1h_in1k)
% \addplot [only marks, mark=otimes*, mark size=4.0, draw=black, mark options={fill=green128}, forget plot]
% table{
%     x y
%     95.8 59.0
% };

% %RN26 in100+oi100 V-Sc
% \addplot [only marks, mark=triangle*, mark size=4.5, draw=black, mark options={fill=blue204}, forget plot]
% table{
%     x y
%     85.8 47.6
% };

%RN50 in100+oi100 V-Sc
\addplot [only marks, mark=triangle*, mark size=2.5, draw=black, mark options={fill=blue128}, forget plot]
table{
    x y
    89.7 50.8
    90.1 51.1
    90.4 51.2
    90.4 51.4
    90.4 51.7
};

% %RN50x4 in100+oi100 V-Sc
% \addplot [only marks, mark=triangle*, mark size=4.5, draw=black, mark options={fill=blue90}, forget plot]
% table{
%     x y
%     90.3 50.1
% };

% %RN26 JANuS V-Sc
% \addplot [only marks, mark=triangle*, mark size=6.0, draw=black, mark options={fill=blue204}, forget plot]
% table{
%     x y
%     86.1 58.0
% };

%RN50 JANuS V-Sc
\addplot [only marks, mark=triangle*, mark size=3.0, draw=black, mark options={fill=blue128}]
table{
    x y
    90.8 65.6
    90.8 66.4
    91.7 66.6
    91.6 67.2
    91.7 67.4
};
\addlegendentry{V-Scaling}

% %RN50x4 JANuS V-Sc
% \addplot [only marks, mark=triangle*, mark size=6.0, draw=black, mark options={fill=blue90}, forget plot]
% table{
%     x y
%     90.9 65.8
% };

%RN50 JANuS+YFCC V-Sc
\addplot [only marks, mark=triangle*, mark size=3.25, draw=black, mark options={fill=blue128}, forget plot]
table{
    x y
    92.5 68.9
    92.7 70.1
    92.7 70.2
};

\addlegendimage{empty legend}
\addlegendentry{(Larger markers $->$ more data)}

% \addlegendimage{empty legend}
% \addlegendentry{(Darker points -> more parameters)}

\end{axis}


\end{tikzpicture}

==> plots/overview_figure.tex <==

\begin{figure}[ht]
  \centering
    % Define the width of the images
  % Define the width of the images
  \newcommand{\myfiguresize}{0.2\textwidth}
  \newcommand{\mylabelsize}{0.1\textwidth}
  
  % Define the space between the figures and subcaptions
  \setlength{\abovecaptionskip}{0.5pt}
  \setlength{\belowcaptionskip}{0.5pt}
  
    \begin{subfigure}[b]{\mylabelsize}
      \caption*{}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{\myfiguresize}
      \caption*{\textbf{ImageNet-1000}}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\myfiguresize}
      \caption*{\textbf{SD-1000}(img2img)}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\myfiguresize}
      \caption*{\textbf{OI-1000}}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\myfiguresize}
      \caption*{\textbf{LA-1000}(img2img)}
    \end{subfigure}
    \vspace{2mm}
  % Row 1: Volcanoes
  % Left side subcaptions (Image categories)
  \begin{subfigure}[b]{\mylabelsize}
      \caption*{\rotatebox{90}{\textbf{Volcano}}}
    \end{subfigure}
    % \hfill
  \begin{subfigure}[t]{\myfiguresize}
    \includegraphics[width=\textwidth]{figures/in1000_v.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{\myfiguresize}
    \includegraphics[width=\textwidth]{figures/sd1000_v.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{\myfiguresize}
    \includegraphics[width=\textwidth]{figures/oi1000_v.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{\myfiguresize}
    \includegraphics[width=\textwidth]{figures/ln1000_v.jpg}
  \end{subfigure}

  % Row 2: School Buses
  \begin{subfigure}[b]{\mylabelsize}
      \caption*{\rotatebox{90}{\textbf{School Bus}}}
    \end{subfigure}
  %\hfill
  \begin{subfigure}[t]{\myfiguresize}
    \includegraphics[width=\textwidth]{figures/in1000_bus.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{\myfiguresize}
    \includegraphics[width=\textwidth]{figures/sd_schoolbus.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{\myfiguresize}
    
    \includegraphics[width=\textwidth]{figures/oi1000_bus.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{\myfiguresize}
    \includegraphics[width=\textwidth]{figures/ln1000_bus.jpg}
  \end{subfigure}

  
  % Row 3: Soccer Balls
  \begin{subfigure}[b]{\mylabelsize}
      \caption*{\rotatebox{90}{\textbf{Soccer}}}
    \end{subfigure}
    % \hfill
  \begin{subfigure}[t]{\myfiguresize}
    \includegraphics[width=\textwidth]{figures/in1000_soccer.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{\myfiguresize}
    \includegraphics[width=\textwidth]{figures/sd_soccur.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{\myfiguresize}
    \includegraphics[width=\textwidth]{figures/oi100_sc.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{\myfiguresize}
    \includegraphics[width=\textwidth]{figures/ln1000_soccer.jpg}
  \end{subfigure}
  
  % Main caption for the entire figure
  \caption{\textbf{Random samples from the ImageNet++ shifts, compared to random samples in the original ImageNet-1k dataset.} The selected classes are "Volcano", "School Bus", and "Soccer". Different viewpoints and centers emerge in these categories of LAION-1k and OI1000. Also, samples generated in SD1000 are illustrations which may defy the laws of physics.}
  \label{fig:datasets_comparison}
\end{figure}



==> tables/datascalingstrategies.tex <==
\begin{table}[!ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
    
        \textbf{Name} & \textbf{D(im, txt) Req'd} & \textbf{Label Set Req'd} & \textbf{Model Req'd} & \textbf{D'(im, txt) Req'd} & \textbf{Experts Req'd} & \textbf{Sample Noise} & \textbf{Imbalance} & \textbf{Cost} & \textbf{Used by} \\
        \midrule
        V-Scaling & No, No & Yes & No & Yes, No & Yes & Low & Low & High & \cite{deng2009imagenet} \\ 
        Crowdsourced Labeling & No, No & Yes & No & Yes, No & Yes & Low & High & High & \cite{kuznetsova2020open} \\ 
        Schema Matching & Yes, Yes & Yes & No & Yes, No & Sometimes & Low & High & Medium & Ours (OI1000) \\ 
        Synthetic img2img & Yes, No & No & Yes & No, No & No & Medium & Low & Medium & Ours (SD1000) \\ 
        Synthetic text2img & No, Yes & Sometimes & Yes & No, No & Sometimes & Medium & Low & Medium & \cite{bansal2023leaving, sariyildiz2023fake, trustless} \\ 
        Embedding Search img2img & Yes, No & Yes & Yes & Yes, No & No & Medium & Low & Medium & Ours (LA1000) \\ 
        Embedding Search text2img & No, Yes & Yes & Yes & Yes, Yes & Sometimes & Medium & Low & Medium & \cite{shirali2023makes} \\ 
        Substring Matching & No, Yes & Yes & No & Yes, Yes & No & Medium & Medium & Low & \cite{feuer2023distributionally} \\ 
        H-Scaling (ours) & No, No & No & No & Yes, No & No & Low & Low & Low & \cite{feuer2023exploring} \\ 
    \end{tabular}}
    \caption{\textbf{Data scaling strategies.} We enumerate the techniques employed for scaling datasets, rank ordered by their approximate costs.}
    \label{tab:scalestrat}
\end{table}

==> tables/tikz/oi1000-100pct.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]
\begin{scope}
    \clip (0,0) rectangle (2,0.2);
    \fill[red] (0,0) rectangle (2,0.2);
    % \fill[green] (1.76,0) rectangle (2,0.2);
\end{scope}
\draw (1,-0.1) -- (1,0.3);
\end{tikzpicture}

==> tables/tikz/oi1000-56pct.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]
\begin{scope}
    \clip (0,0) rectangle (2,0.2);
    \fill[red] (0,0) rectangle (1.12,0.2);
    \fill[green] (1.12,0) rectangle (2,0.2);
\end{scope}
\draw (1,-0.1) -- (1,0.3);
\end{tikzpicture}

==> tables/tikz/oi1000-88pct.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]
\begin{scope}
    \clip (0,0) rectangle (2,0.2);
    \fill[red] (0,0) rectangle (1.76,0.2);
    \fill[green] (1.76,0) rectangle (2,0.2);
\end{scope}
\draw (1,-0.1) -- (1,0.3);
\end{tikzpicture}
